Gravitational Infall onto Molecular Filaments II. Externally Pressurized Cylinders

In an extension of Fischera & Martin (2012a) and Heitsch (2013), two aspects of the evolution of externally pressurized, hydrostatic filaments are discussed. (a) The free-fall accretion of gas onto such a filament will lead to filament parameters (specifically, FWHM--column density relations) inconsistent with the observations of Arzoumanian et al. (2011), except for two cases: For low-mass, isothermal filaments, agreement is found as in the analysis by Fischera & Martin (2012b). Magnetized cases, for which the field scales weakly with the density as $B\propto n^{1/2}$, also reproduce observed parameters. (b) Realistically, the filaments will be embedded not only in gas of non-zero pressure, but also of non-zero density. Thus, the appearance of sheet-embedded filaments is explored. Generating a grid of filament models and comparing the resulting column density ratios and profile shapes with observations suggests that the three-dimensional filament profiles are intrinsically flatter than isothermal, beyond projection and evolution effects.

==> journal.tex <==
\newcommand{\apj}    {ApJ}
\newcommand{\apjs}   {ApJS}
\newcommand{\apjl}   {ApJL}
\newcommand{\aj}     {AJ}
\newcommand{\mnras}  {MNRAS}
\newcommand{\aap}    {A\&A}
\newcommand{\aaps}   {A\&AS}
\newcommand{\araa}   {ARAA}
\newcommand{\nat}    {Nature}
\newcommand{\pasj}   {PASJ}
\newcommand{\pasp}   {PASP}
\newcommand{\apss}   {ApSS}
\newcommand{\phfl}   {Phys. Fl.}
\newcommand{\phrev}  {Phys. Rev.}
\newcommand{\pre}    {Phys. Rev. E}
\newcommand{\jcp}    {J. Comp. Phys.}
\newcommand{\qjras}  {Quart. Jour. of the R.~ A.~S.}
\newcommand{\grl}    {Geophys. Rev. Lett.}


